An Accelerated Gradient Method for Convex Smooth Simple Bilevel Optimization

In this paper, we focus on simple bilevel optimization problems, where we minimize a convex smooth objective function over the optimal solution set of another convex smooth constrained optimization problem. We present a novel bilevel optimization method that locally approximates the solution set of the lower-level problem using a cutting plane approach and employs an accelerated gradient-based update to reduce the upper-level objective function over the approximated solution set. We measure the performance of our method in terms of suboptimality and infeasibility errors and provide non-asymptotic convergence guarantees for both error criteria. Specifically, when the feasible set is compact, we show that our method requires at most $\mathcal{O}(\max\{1/\sqrt{\epsilon_{f}}, 1/\epsilon_g\})$ iterations to find a solution that is $\epsilon_f$-suboptimal and $\epsilon_g$-infeasible. Moreover, under the additional assumption that the lower-level objective satisfies the $r$-th H\"olderian error bound, we show that our method achieves an iteration complexity of $\mathcal{O}(\max\{\epsilon_{f}^{-\frac{2r-1}{2r}},\epsilon_{g}^{-\frac{2r-1}{2r}}\})$, which matches the optimal complexity of single-level convex constrained optimization when $r=1$.

==> math_commands.tex <==
% Adapted for use with thuthesis.
% Original code is at https://github.com/goodfeli/dlbook_notation/blob/master/math_commands.tex

%%%%% NEW MATH DEFINITIONS %%%%%

\newcommand\ceil[1]{\lceil #1 \rceil}
\newcommand\floor[1]{\lfloor #1 \rfloor}


% Vectors
% \newcommand\Vector[1]{\symbf{#1}}
\newcommand\Vector[1]{\mathbf{#1}}

\newcommand\0{{\Vector{0}}}
\newcommand\vzero{{\Vector{0}}}
\newcommand\1{{\Vector{1}}}
\newcommand\vone{{\Vector{1}}}

\newcommand\va{{\Vector{a}}}
\newcommand\vb{{\Vector{b}}}
\newcommand\vc{{\Vector{c}}}
\newcommand\vd{{\Vector{d}}}
\newcommand\ve{{\Vector{e}}}
\newcommand\vf{{\Vector{f}}}
\newcommand\vg{{\Vector{g}}}
\newcommand\vh{{\Vector{h}}}
\newcommand\vi{{\Vector{i}}}
\newcommand\vj{{\Vector{j}}}
\newcommand\vk{{\Vector{k}}}
\newcommand\vl{{\Vector{l}}}
\newcommand\vm{{\Vector{m}}}
\newcommand\vn{{\Vector{n}}}
\newcommand\vo{{\Vector{o}}}
\newcommand\vp{{\Vector{p}}}
\newcommand\vq{{\Vector{q}}}
\newcommand\vr{{\Vector{r}}}
\newcommand\vs{{\Vector{s}}}
\newcommand\vt{{\Vector{t}}}
\newcommand\vu{{\Vector{u}}}
\newcommand\vv{{\Vector{v}}}
\newcommand\vw{{\Vector{w}}}
\newcommand\vx{{\Vector{x}}}
\newcommand\vy{{\Vector{y}}}
\newcommand\vz{{\Vector{z}}}

\newcommand\valpha{{\Vector{\alpha}}}
\newcommand\vbeta{{\Vector{\beta}}}
\newcommand\vgamma{{\Vector{\gamma}}}
\newcommand\vdelta{{\Vector{\delta}}}
\newcommand\vepsilon{{\Vector{\epsilon}}}
\newcommand\vtheta{{\Vector{\theta}}}
\newcommand\viota{{\Vector{\iota}}}
\newcommand\vkappa{{\Vector{\kappa}}}
\newcommand\vlambda{{\Vector{\lambda}}}
\newcommand\vmu{{\Vector{\mu}}}
\newcommand\vnu{{\Vector{\nu}}}
\newcommand\vxi{{\Vector{\xi}}}
\newcommand\vpi{{\Vector{\pi}}}
\newcommand\vrho{{\Vector{\rho}}}
\newcommand\vsigma{{\Vector{\sigma}}}
\newcommand\vtau{{\Vector{\tau}}}
\newcommand\vupsilon{{\Vector{\upsilon}}}
\newcommand\vphi{{\Vector{\phi}}}
\newcommand\vchi{{\Vector{\chi}}}
\newcommand\vpsi{{\Vector{\psi}}}
\newcommand\vomega{{\Vector{\omega}}}
\newcommand\veta{{\Vector{\eta}}}

\newcommand\vha{{\hat{\Vector{a}}}}
\newcommand\vhb{{\hat{\Vector{b}}}}
\newcommand\vhc{{\hat{\Vector{c}}}}
\newcommand\vhd{{\hat{\Vector{d}}}}
\newcommand\vhe{{\hat{\Vector{e}}}}
\newcommand\vhf{{\hat{\Vector{f}}}}
\newcommand\vhg{{\hat{\Vector{g}}}}
\newcommand\vhh{{\hat{\Vector{h}}}}
\newcommand\vhi{{\hat{\Vector{i}}}}
\newcommand\vhj{{\hat{\Vector{j}}}}
\newcommand\vhk{{\hat{\Vector{k}}}}
\newcommand\vhl{{\hat{\Vector{l}}}}
\newcommand\vhm{{\hat{\Vector{m}}}}
\newcommand\vhn{{\hat{\Vector{n}}}}
\newcommand\vho{{\hat{\Vector{o}}}}
\newcommand\vhp{{\hat{\Vector{p}}}}
\newcommand\vhq{{\hat{\Vector{q}}}}
\newcommand\vhr{{\hat{\Vector{r}}}}
\newcommand\vhs{{\hat{\Vector{s}}}}
\newcommand\vht{{\hat{\Vector{t}}}}
\newcommand\vhu{{\hat{\Vector{u}}}}
\newcommand\vhv{{\hat{\Vector{v}}}}
\newcommand\vhw{{\hat{\Vector{w}}}}
\newcommand\vhx{{\hat{\Vector{x}}}}
\newcommand\vhy{{\hat{\Vector{y}}}}
\newcommand\vhz{{\hat{\Vector{z}}}}
% Matrix
% \newcommand\MATRIX[1]{\symbf{#1}}
\newcommand\MATRIX[1]{\mathbf{#1}}

\newcommand\mA{{\MATRIX{A}}}
\newcommand\mB{{\MATRIX{B}}}
\newcommand\mC{{\MATRIX{C}}}
\newcommand\mD{{\MATRIX{D}}}
\newcommand\mE{{\MATRIX{E}}}
\newcommand\mF{{\MATRIX{F}}}
\newcommand\mG{{\MATRIX{G}}}
\newcommand\mH{{\MATRIX{H}}}
\newcommand\mI{{\MATRIX{I}}}
\newcommand\mJ{{\MATRIX{J}}}
\newcommand\mK{{\MATRIX{K}}}
\newcommand\mL{{\MATRIX{L}}}
\newcommand\mM{{\MATRIX{M}}}
\newcommand\mN{{\MATRIX{N}}}
\newcommand\mO{{\MATRIX{O}}}
\newcommand\mP{{\MATRIX{P}}}
\newcommand\mQ{{\MATRIX{Q}}}
\newcommand\mR{{\MATRIX{R}}}
\newcommand\mS{{\MATRIX{S}}}
\newcommand\mT{{\MATRIX{T}}}
\newcommand\mU{{\MATRIX{U}}}
\newcommand\mV{{\MATRIX{V}}}
\newcommand\mW{{\MATRIX{W}}}
\newcommand\mX{{\MATRIX{X}}}
\newcommand\mY{{\MATRIX{Y}}}
\newcommand\mZ{{\MATRIX{Z}}}

\newcommand\mhA{{\hat{\MATRIX{A}}}}
\newcommand\mhB{{\hat{\MATRIX{B}}}}
\newcommand\mhC{{\hat{\MATRIX{C}}}}
\newcommand\mhD{{\hat{\MATRIX{D}}}}
\newcommand\mhE{{\hat{\MATRIX{E}}}}
\newcommand\mhF{{\hat{\MATRIX{F}}}}
\newcommand\mhG{{\hat{\MATRIX{G}}}}
\newcommand\mhH{{\hat{\MATRIX{H}}}}
\newcommand\mhI{{\hat{\MATRIX{I}}}}
\newcommand\mhJ{{\hat{\MATRIX{J}}}}
\newcommand\mhK{{\hat{\MATRIX{K}}}}
\newcommand\mhL{{\hat{\MATRIX{L}}}}
\newcommand\mhM{{\hat{\MATRIX{M}}}}
\newcommand\mhN{{\hat{\MATRIX{N}}}}
\newcommand\mhO{{\hat{\MATRIX{O}}}}
\newcommand\mhP{{\hat{\MATRIX{P}}}}
\newcommand\mhQ{{\hat{\MATRIX{Q}}}}
\newcommand\mhR{{\hat{\MATRIX{R}}}}
\newcommand\mhS{{\hat{\MATRIX{S}}}}
\newcommand\mhT{{\hat{\MATRIX{T}}}}
\newcommand\mhU{{\hat{\MATRIX{U}}}}
\newcommand\mhV{{\hat{\MATRIX{V}}}}
\newcommand\mhW{{\hat{\MATRIX{W}}}}
\newcommand\mhX{{\hat{\MATRIX{X}}}}
\newcommand\mhY{{\hat{\MATRIX{Y}}}}
\newcommand\mhZ{{\hat{\MATRIX{Z}}}}

\newcommand\mGamma{{\MATRIX{\Gamma}}}
\newcommand\mDelta{{\MATRIX{\Delta}}}
\newcommand\mTheta{{\MATRIX{\Theta}}}
\newcommand\mLambda{{\MATRIX{\Lambda}}}
\newcommand\mXi{{\MATRIX{\Xi}}}
\newcommand\mPi{{\MATRIX{\Pi}}}
\newcommand\mSigma{{\MATRIX{\Sigma}}}
\newcommand\mUpsilon{{\MATRIX{\Upsilon}}}
\newcommand\mPhi{{\MATRIX{\Phi}}}
\newcommand\mPsi{{\MATRIX{\Psi}}}
\newcommand\mOmega{{\MATRIX{\Omega}}}


% Tensor
% \newcommand\tens[1]{\symbfsf{#1}}
% \newcommand\tA{{\tens{A}}}
% \newcommand\tB{{\tens{B}}}
% \newcommand\tC{{\tens{C}}}
% \newcommand\tD{{\tens{D}}}
% \newcommand\tE{{\tens{E}}}
% \newcommand\tF{{\tens{F}}}
% \newcommand\tG{{\tens{G}}}
% \newcommand\tH{{\tens{H}}}
% \newcommand\tI{{\tens{I}}}
% \newcommand\tJ{{\tens{J}}}
% \newcommand\tK{{\tens{K}}}
% \newcommand\tL{{\tens{L}}}
% \newcommand\tM{{\tens{M}}}
% \newcommand\tN{{\tens{N}}}
% \newcommand\tO{{\tens{O}}}
% \newcommand\tP{{\tens{P}}}
% \newcommand\tQ{{\tens{Q}}}
% \newcommand\tR{{\tens{R}}}
% \newcommand\tS{{\tens{S}}}
% \newcommand\tT{{\tens{T}}}
% \newcommand\tU{{\tens{U}}}
% \newcommand\tV{{\tens{V}}}
% \newcommand\tW{{\tens{W}}}
% \newcommand\tX{{\tens{X}}}
% \newcommand\tY{{\tens{Y}}}
% \newcommand\tZ{{\tens{Z}}}


% Graph
\newcommand\gA{{\mathcal{A}}}
\newcommand\gB{{\mathcal{B}}}
\newcommand\gC{{\mathcal{C}}}
\newcommand\gD{{\mathcal{D}}}
\newcommand\gE{{\mathcal{E}}}
\newcommand\gF{{\mathcal{F}}}
\newcommand\gG{{\mathcal{G}}}
\newcommand\gH{{\mathcal{H}}}
\newcommand\gI{{\mathcal{I}}}
\newcommand\gJ{{\mathcal{J}}}
\newcommand\gK{{\mathcal{K}}}
\newcommand\gL{{\mathcal{L}}}
\newcommand\gM{{\mathcal{M}}}
\newcommand\gN{{\mathcal{N}}}
\newcommand\gO{{\mathcal{O}}}
\newcommand\gP{{\mathcal{P}}}
\newcommand\gQ{{\mathcal{Q}}}
\newcommand\gR{{\mathcal{R}}}
\newcommand\gS{{\mathcal{S}}}
\newcommand\gT{{\mathcal{T}}}
\newcommand\gU{{\mathcal{U}}}
\newcommand\gV{{\mathcal{V}}}
\newcommand\gW{{\mathcal{W}}}
\newcommand\gX{{\mathcal{X}}}
\newcommand\gY{{\mathcal{Y}}}
\newcommand\gZ{{\mathcal{Z}}}


% Sets
\newcommand\sA{{\mathbb{A}}}
\newcommand\sB{{\mathbb{B}}}
\newcommand\sC{{\mathbb{C}}}
\newcommand\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\newcommand\sF{{\mathbb{F}}}
\newcommand\sG{{\mathbb{G}}}
\newcommand\sH{{\mathbb{H}}}
\newcommand\sI{{\mathbb{I}}}
\newcommand\sJ{{\mathbb{J}}}
\newcommand\sK{{\mathbb{K}}}
\newcommand\sL{{\mathbb{L}}}
\newcommand\sM{{\mathbb{M}}}
\newcommand\sN{{\mathbb{N}}}
\newcommand\sO{{\mathbb{O}}}
\newcommand\sP{{\mathbb{P}}}
\newcommand\sQ{{\mathbb{Q}}}
\newcommand\sR{{\mathbb{R}}}
\newcommand\sS{{\mathbb{S}}}
\newcommand\sT{{\mathbb{T}}}
\newcommand\sU{{\mathbb{U}}}
\newcommand\sV{{\mathbb{V}}}
\newcommand\sW{{\mathbb{W}}}
\newcommand\sX{{\mathbb{X}}}
\newcommand\sY{{\mathbb{Y}}}
\newcommand\sZ{{\mathbb{Z}}}

\renewcommand\sA{{\mathcal{A}}}
\renewcommand\sS{{\mathcal{S}}}
\renewcommand\sQ{{\mathcal{Q}}}

% Random variables
\newcommand\RandomVariable[1]{\symit{#1}}

\newcommand\rA{{\RandomVariable{A}}}
\newcommand\rB{{\RandomVariable{B}}}
\newcommand\rC{{\RandomVariable{C}}}
\newcommand\rD{{\RandomVariable{D}}}
\newcommand\rE{{\RandomVariable{E}}}
\newcommand\rF{{\RandomVariable{F}}}
\newcommand\rG{{\RandomVariable{G}}}
\newcommand\rH{{\RandomVariable{H}}}
\newcommand\rI{{\RandomVariable{I}}}
\newcommand\rJ{{\RandomVariable{J}}}
\newcommand\rK{{\RandomVariable{K}}}
\newcommand\rL{{\RandomVariable{L}}}
\newcommand\rM{{\RandomVariable{M}}}
\newcommand\rN{{\RandomVariable{N}}}
\newcommand\rO{{\RandomVariable{O}}}
\newcommand\rP{{\RandomVariable{P}}}
\newcommand\rQ{{\RandomVariable{Q}}}
\newcommand\rR{{\RandomVariable{R}}}
\newcommand\rS{{\RandomVariable{S}}}
\newcommand\rT{{\RandomVariable{T}}}
\newcommand\rU{{\RandomVariable{U}}}
\newcommand\rV{{\RandomVariable{V}}}
\newcommand\rW{{\RandomVariable{W}}}
\newcommand\rX{{\RandomVariable{X}}}
\newcommand\rY{{\RandomVariable{Y}}}
\newcommand\rZ{{\RandomVariable{Z}}}

% Random vectors
\newcommand\RandomVector[1]{\symbf{#1}}

\newcommand\rvA{{\RandomVector{A}}}
\newcommand\rvB{{\RandomVector{B}}}
\newcommand\rvC{{\RandomVector{C}}}
\newcommand\rvD{{\RandomVector{D}}}
\newcommand\rvE{{\RandomVector{E}}}
\newcommand\rvF{{\RandomVector{F}}}
\newcommand\rvG{{\RandomVector{G}}}
\newcommand\rvH{{\RandomVector{H}}}
\newcommand\rvI{{\RandomVector{I}}}
\newcommand\rvJ{{\RandomVector{J}}}
\newcommand\rvK{{\RandomVector{K}}}
\newcommand\rvL{{\RandomVector{L}}}
\newcommand\rvM{{\RandomVector{M}}}
\newcommand\rvN{{\RandomVector{N}}}
\newcommand\rvO{{\RandomVector{O}}}
\newcommand\rvP{{\RandomVector{P}}}
\newcommand\rvQ{{\RandomVector{Q}}}
\newcommand\rvR{{\RandomVector{R}}}
\newcommand\rvS{{\RandomVector{S}}}
\newcommand\rvT{{\RandomVector{T}}}
\newcommand\rvU{{\RandomVector{U}}}
\newcommand\rvV{{\RandomVector{V}}}
\newcommand\rvW{{\RandomVector{W}}}
\newcommand\rvX{{\RandomVector{X}}}
\newcommand\rvY{{\RandomVector{Y}}}
\newcommand\rvZ{{\RandomVector{Z}}}

% Vectors

\newcommand\ba{{\bar{a}}}
\newcommand\bb{{\bar{b}}}
\newcommand\bc{{\bar{c}}}
\newcommand\bd{{\bar{d}}}
\newcommand\be{{\bar{e}}}

\newcommand\bg{{\bar{g}}}
\newcommand\bh{{\bar{h}}}
\newcommand\bi{{\bar{i}}}
\newcommand\bj{{\bar{j}}}
\newcommand\bk{{\bar{k}}}
\newcommand\bl{{\bar{l}}}

\newcommand\bn{{\bar{n}}}
\newcommand\bo{{\bar{o}}}
\newcommand\bp{{\bar{p}}}
\newcommand\bq{{\bar{q}}}
% \newcommand\br{{\bar{r}}}
\newcommand\bs{{\bar{s}}}
\newcommand\bt{{\bar{t}}}
\newcommand\bu{{\bar{u}}}
\newcommand\bv{{\bar{v}}}
\newcommand\bw{{\bar{w}}}
\newcommand\bx{{\bar{x}}}
\newcommand\by{{\bar{y}}}
\newcommand\bz{{\bar{z}}}

\newcommand\balpha{{\bar{\alpha}}}
\newcommand\bbeta{{\bar{\beta}}}
\newcommand\bgamma{{\bar{\gamma}}}
\newcommand\bdelta{{\bar{\delta}}}
\newcommand\bepsilon{{\bar{\epsilon}}}
\newcommand\btheta{{\bar{\theta}}}
\newcommand\biota{{\bar{\iota}}}
\newcommand\bkappa{{\bar{\kappa}}}
\newcommand\blambda{{\bar{\lambda}}}
\newcommand\bmu{{\bar{\mu}}}
\newcommand\bnu{{\bar{\nu}}}
\newcommand\bxi{{\bar{\xi}}}
\newcommand\bpi{{\bar{\pi}}}
\newcommand\brho{{\bar{\rho}}}
\newcommand\bsigma{{\bar{\sigma}}}
\newcommand\btau{{\bar{\tau}}}
\newcommand\bupsilon{{\bar{\upsilon}}}
\newcommand\bphi{{\bar{\phi}}}
\newcommand\bchi{{\bar{\chi}}}
\newcommand\bpsi{{\bar{\psi}}}
\newcommand\bomega{{\bar{\omega}}}

\newcommand\bA{{\bar{A}}}
\newcommand\bB{{\bar{B}}}
\newcommand\bC{{\bar{C}}}
\newcommand\bD{{\bar{D}}}
\newcommand\bF{{\bar{F}}}
\newcommand\bG{{\bar{G}}}
\newcommand\bH{{\bar{H}}}
\newcommand\bI{{\bar{I}}}
\newcommand\bJ{{\bar{J}}}
\newcommand\bK{{\bar{K}}}
\newcommand\bL{{\bar{L}}}
\newcommand\bM{{\bar{M}}}
\newcommand\bN{{\bar{N}}}
\newcommand\bO{{\bar{O}}}
\newcommand\bP{{\bar{P}}}
\newcommand\bQ{{\bar{Q}}}
\newcommand\bR{{\bar{R}}}
\newcommand\bS{{\bar{S}}}
\newcommand\bT{{\bar{T}}}
\newcommand\bU{{\bar{U}}}
\newcommand\bV{{\bar{V}}}
\newcommand\bW{{\bar{W}}}
\newcommand\bX{{\bar{X}}}
\newcommand\bY{{\bar{Y}}}
\newcommand\bZ{{\bar{Z}}}
\newcommand\bLambda{{\bar{\Lambda}}}
\newcommand\bGamma{{\bar{\Gamma}}}

% bv
\newcommand\bva{{\bar{\va}}}
\newcommand\bvb{{\bar{\vb}}}
\newcommand\bvc{{\bar{\vc}}}
\newcommand\bvd{{\bar{\vd}}}
\newcommand\bve{{\bar{\ve}}}

\newcommand\bvg{{\bar{\vg}}}
\newcommand\bvh{{\bar{\vh}}}
\newcommand\bvi{{\bar{\vi}}}
\newcommand\bvj{{\bar{\vj}}}
\newcommand\bvk{{\bar{\vk}}}
\newcommand\bvl{{\bar{\vl}}}

\newcommand\bvn{{\bar{\vn}}}
\newcommand\bvo{{\bar{\vo}}}
\newcommand\bvp{{\bar{\vp}}}
\newcommand\bvq{{\bar{\vq}}}
\newcommand\bvr{{\bar{\vr}}}
\newcommand\bvs{{\bar{\vs}}}
\newcommand\bvt{{\bar{\vt}}}
\newcommand\bvu{{\bar{\vu}}}
\newcommand\bvv{{\bar{\vv}}}
\newcommand\bvw{{\bar{\vw}}}
\newcommand\bvx{{\bar{\vx}}}
\newcommand\bvy{{\bar{\vy}}}
\newcommand\bvz{{\bar{\vz}}}

\newcommand\bvalpha{{\bar{\valpha}}}
\newcommand\bvbeta{{\bar{\vbeta}}}
\newcommand\bvgamma{{\bar{\vgamma}}}
\newcommand\bvdelta{{\bar{\vdelta}}}
\newcommand\bvepsilon{{\bar{\vepsilon}}}
\newcommand\bvtheta{{\bar{\vtheta}}}
\newcommand\bviota{{\bar{\viota}}}
\newcommand\bvkappa{{\bar{\vkappa}}}
\newcommand\bvlambda{{\bar{\vlambda}}}
\newcommand\bvmu{{\bar{\vmu}}}
\newcommand\bvnu{{\bar{\vnu}}}
\newcommand\bvxi{{\bar{\vxi}}}
\newcommand\bvpi{{\bar{\vpi}}}
\newcommand\bvrho{{\bar{\vrho}}}
\newcommand\bvsigma{{\bar{\vsigma}}}
\newcommand\bvtau{{\bar{\vtau}}}
\newcommand\bvupsilon{{\bar{\vupsilon}}}
\newcommand\bvphi{{\bar{\vphi}}}
\newcommand\bvchi{{\bar{\vchi}}}
\newcommand\bvpsi{{\bar{\vpsi}}}
\newcommand\bvomega{{\bar{\vomega}}}

% \newcommand\bvA{{\bar{A}}}
% \newcommand\bvB{{\bar{B}}}
% \newcommand\bvC{{\bar{C}}}
% \newcommand\bvD{{\bar{D}}}
% \newcommand\bvF{{\bar{F}}}
% \newcommand\bvG{{\bar{G}}}
% \newcommand\bvH{{\bar{H}}}
% \newcommand\bvI{{\bar{I}}}
% \newcommand\bvJ{{\bar{J}}}
% \newcommand\bvK{{\bar{K}}}
% \newcommand\bvL{{\bar{L}}}
\newcommand\bmM{{\bar{\mM}}}
% \newcommand\bvN{{\bar{N}}}
% \newcommand\bvO{{\bar{O}}}
% \newcommand\bvP{{\bar{P}}}
% \newcommand\bvQ{{\bar{Q}}}
% \newcommand\bvR{{\bar{R}}}
% \newcommand\bvS{{\bar{S}}}
% \newcommand\bvT{{\bar{T}}}
% \newcommand\bvU{{\bar{U}}}
% \newcommand\bvV{{\bar{V}}}
% \newcommand\bvW{{\bar{W}}}
% \newcommand\bvX{{\bar{X}}}
% \newcommand\bvY{{\bar{Y}}}
% \newcommand\bvZ{{\bar{Z}}}
\newcommand\bmLambda{{\bar{\mLambda}}}
\newcommand\bmGamma{{\bar{\mGamma}}}



\newcommand\tlambda{{\tilde{\lambda}}}
\newcommand\tLambda{{\tilde{\Lambda}}}

\newcommand\tmu{{\tilde{\mu}}}

\newcommand\laplace{\mathrm{Laplace}} % Laplace distribution

\newcommand\bigO{\mathcal{O}}
\newcommand\semiS[1]{{\mathbb{S}_{+}^{#1}}}
\newcommand\Prob{\mathbf{Prob}}
% \newcommand\I{\mathbb{I}} % Indicator function
\newcommand\givenp[1][]{{\:#1\vert\:}}
\newcommand\Diag{{\mathrm{Diag}}}
\newcommand\Real{{\mathrm{Re}}}
\newcommand\Imag{{\mathrm{Im}}}
\DeclareMathOperator*{\E}{\mathbb{E}}
% \newcommand\E{\mathbb{E}}
\newcommand\Ls{\mathcal{L}}
% \newcommand\R{\mathbb{R}}
% \newcommand\C{\mathbb{C}}
\newcommand\emp{\tilde{p}}
\newcommand\lr{\alpha}
\newcommand\reg{\lambda}
\newcommand\rect{\mathrm{rectifier}}
\newcommand\softmax{\mathrm{softmax}}
\newcommand\sigmoid{\sigma}
\newcommand\softplus{\zeta}
\newcommand\KL{D_{\mathrm{KL}}}
\newcommand\Var{\mathrm{Var}}
\newcommand\standarderror{\mathrm{SE}}
\newcommand\Cov{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand\normlzero{L^0}
\newcommand\normlone{L^1}
\newcommand\normltwo{L^2}
\newcommand\normlp{L^p}
\newcommand\normmax{L^\infty}
\newcommand\imag{{\mathbf{i}}}
% \newcommand\T{{\mathsf{T}}}
\newcommand\op{{\mathrm{op}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\interior}{int\,}
\DeclareMathOperator{\dom}{dom\,}
\let\ab\allowbreak

